High Power Cyclotrons: The Bridge Between Beyond the Standard Model Physics, Computation, and Medical Applications

The IsoDAR cyclotron is a 60 MeV cyclotron designed to output 10mA of protons in order to be a driver for a neutrino experiment. Coupling the high flux generated by the IsoDAR system with a kiloton neutrino detector will provide sterile neutrino exclusion searches covering anomalous regions indicated by short baseline experiments. Simultaneously, the coupling of a high power target and kiloton detector allows for the investigation of dark matter candidates, namely axion-like particles. We have shown that nuclear excitations within the IsoDAR target create a unique opportunity to produce axions and detect monoenergetic peaks with the nearby kiloton detector. Beyond this, the high power produced by the IsoDAR cyclotron can be used for applications beyond particle physics. The IsoDAR cyclotron accelerates and extracts H$_2^+$, which allows the beam to be split downstream, a versatile and important development to alleviate the problem of producing high-power targets for the medical isotope community. This thesis presents a proposal for production of an more than an order of magnitude higher rates than are available at present for certain highly-need medical isotopes, including Ac-225. In this thesis, we report results from a multi-cusp ion source that meets these requirements and produces a record level of high purity, low emittance H$_2^+$ current. The second has been to design a radio-frequency quadrupole (RFQ) that will allow for gentle bunching of the high current before injection. This is the first use of axial direct injection with a compact cyclotron. This thesis reports the first application of machine learning to the RFQ design. These tools enable the high currents required by IsoDAR cyclotron, leading to important impact on the accelerator, medical, and physics communities.

==> READMEs/README_bibliography.tex <==
%% This file gives an overview on what you will need to do to create a
%% bibliographic database for references, as well as create the actual
%% bibliography for your thesis.

%% You should not need to touch the file biblio.tex.  This merely tells
%% latex to look for the file with the bibliographic info.  The file you
%% want to edit is main.bib.  For each entry, use the appropriate style
%% as designated in the file.

%% Citing your references:

%% When you cite a reference, you need to use the ``key'' you declare in
%% main.bib for the entry.  No one ever sees the keys, but you'll want to
%% use something you will easily remember.  For instance, if you had an
%% entry with:

%% 	   key=geer1

%% Then you would use \cite{geer1} to reference it within your thesis.

%% NOTE: You can not include references in your bibliography that are
%% never cited in your paper by default. If you need to do this, create a
%% key for the entry and at the end of your thesis include the line:

%% \nocite{key}

%% This should be done for every entry which is not explicitly cited.



==> READMEs/README_main.tex <==
%% This file explains the options available to you for editing the file
%% main.tex.

%% The commands in this file allow you to specify options such as
%% spacing, double-sided printing, a draft copy, etc.   By default, 12pt
%% and lgrind are included; lgrind is the 2e style for including code in
%% your thesis.

%% \documentclass[12pt]{mitthesis}
%% \usepackage{lgrind}
%% \pagestyle{plain}

%% You can add options in the documentclass line as follows:

%% 	o  singlespace
%% 	\documentclass[12pt,singlespace]{mitthesis}
	
%% 	o  twoside
%% 	\documentclass[12pt,twoside]{mitthesis}

%% 	o  draft   (make sure to change the pagestyle to drafthead as well)
%% 	\documentclass[12pt,draft]{mitthesis}
%% 	\usepackage{lgrind}
%% 	\pagestyle{drafthead}

%% 	o vi   (for course vi and course viii theses)
%% 	\documentclass[12pt,vi]{mitthesis}

%% Any options you would use for report.sty will work here as well.


%% You should not need to change the first three lines and last two lines
%% below.  Be sure to include an \include command for each file you are
%% including in your thesis.
  
%% \include{cover}
%% \pagestyle{plain}
%% \include{contents}
%% \include{chap1}
%% \include{chap2}
%% \appendix
%% \include{appa}
%% \include{appb}
%% \include{biblio}
%% \end{document}

%% Comment: to include appendices use a single \appendix command followed 
%% by a number of \include{} commands as many files as needed, each of 
%% which should contain a \chapter{} command for the appendix title.


==> READMEs/README_text.tex <==
%% This file includes the basic commands you will need to use within each
%% chapter of your thesis.

%% The file chap1.tex is a sample first chapter.  To get started, you may
%% just want to replace the text and commands in that file as needed.  In
%% general though, for each new chapter you want to do the following:

%% 	o Make sure the name has the extension .tex .  Otherwise, you
%% 	can call it anything you want.  For ease of use, all the
%% 	examples use chap1, chap2, etc.

%% 	o Add a line to the file main.tex that reads:
%% 	\include{yourfilename}

%% 	This should not include the .tex extension, because latex
%% 	assumes that is there.

%% Basic syntax:

%% 	o The first line of each chapter should be:
%% 	\chapter{Chapter Title}

%% 	o To start a new section (labeled chap#.sec# -- as in 1.1,
%% 	1.2, etc):
%% 	\section{Section Heading}

%% 	You can also include subsections:
%% 	\subsection{Heading}




==> appc.tex <==



\chapter{Discussion of Cyclotron Design}


I work within a collaboration of approximately 30 people 
\includepdf[pages={-}]{NIM.pdf}
%\includepdf[pages={-}]{IsoDAR_cdr.pdf}


\clearpage
\newpage

